A Graph-Based Approach to Generate Energy-Optimal Robot Trajectories in Polygonal Environments

As robotic systems continue to address emerging issues in areas such as logistics, mobility, manufacturing, and disaster response, it is increasingly important to rapidly generate safe and energy-efficient trajectories. In this article, we present a new approach to plan energy-optimal trajectories through cluttered environments containing polygonal obstacles. In particular, we develop a method to quickly generate optimal trajectories for a double-integrator system, and we show that optimal path planning reduces to an integer program. To find an efficient solution, we present a distance-informed prefix search to efficiently generate optimal trajectories for a large class of environments. We demonstrate that our approach, while matching the performance of RRT* and Probabilistic Road Maps in terms of path length, outperforms both in terms of energy cost and computational time by up to an order of magnitude. We also demonstrate that our approach yields implementable trajectories in an experiment with a Crazyflie quadrotor.

==> preamble/.git/objects/21/71de1b239b0628e4fad73fd8e7387838b4e8b6 <==
x•ŽÁmÃ0E{Ö\ EK²AÈ¥è¢I¢+Pèýktƒ^þå῵?›Mé͇*`1BSi'—œI"IbÎE+gLQg[D×¼"gº;ÌLy²)U–V°åZç"I‰*	a6,Ó›rh‡÷Ÿux‡¯Ñw¸úÉ>ÞUŽÄR0á‰
—s`XÿÚ\ÿg…{—Í6µvü8ô§o}ÿëP¿
ÊJi

==> preamble/.git/objects/3b/8c51062d3f6f0205cd539db347509272a7489f <==
x•ŽMjÃ0F»Ö)æ-ÒH²-(!½Bé¾h~"š(Ècèñkrƒl>Þâ=ø¸_¯«FÿbC*bËEœ&Â%#ê\%äLmN-GMêKJLî^‡Þ¤H@OS
ÚR\˜1Ò!©¢SãÒBEvu·Ÿ>೓ëð5ú
ÞíØ3ío*û	Â4ùäç¼à?¾™>W¹ •~«éß÷¶_.ºl<Ö»¹gæJW

==> preamble/.git/objects/cc/56792400e4c8561cb5b33079d8851ac18634e8 <==
xuTQkÜ0Þ³¡ÿApo8=è^¶§ën…²ŽÞ­ŒR8GI¼Ø±±kӇýöÉIÖÂؽ8',}'>É)µ-a½¾ºúÀ·ûã>ZŒoœÓ¸µC©I¹ÝߝÐ{U!c+¸'¶3"ØWð¬bñÙ"géæâ"ùÚÁ"½P:0~̒e§4ˆ­ˆ`TÓFΡð z2"xk#Øœ¬%ÝZIß>ÞãIeû?¬//¯žÈ*Æ÷ÎFÀ–«g½ðãMDC™^"Ix˜0Sy\É>¤z¶Ê£¤^UE0"¨"Ö#H"bÔ£GC°Ù}‡ÐŠwV®ÿ҃¡‹Ö±oHýû¦t°³ºBÏÞj¥á*:ʜg9[á'hTTMO|NF–ýfO«ìiÅ
ŽFÈÀ«%Á?:×Vv,ã¨%C´y'̵
'E/Œcœ`Rw¾ÉS&Æ-IªÊ)PÄÄ%ˎÂËV¦‰Öz4¢ÃÙ7;.*Ÿ0Ôê4>VÌZÑR.ëÇ7]‹+åSNÔN€²Í@j'ìëˆ/NÆ=êdÝüørÀŸº€z&®HJÁ²lÈKŠÐ½cò¤ŒØŒòN²Eb"êž"c¢&¡ô´·	½*oš7=›§Xçí/2O»9·ÈßMŒÓMš—·Áý´å®ªoÕNsHNÃË|.ӉVž	½VåX–šBJ}.Ç~ìe;»‰?Þ¼ž½Ç:1IÏékÚÂ](þOíÕ=¾Dô½ÐêuZ	
0ÕG:+Û39¨giMz"äg‡tNœq–ô‡°frÌÜã£roðª\2§ïŸxø

==> preamble/.git/objects/ec/32f072e04528eb63aa88bef625b28ed7d38d48 <==
x•Ž[jÄ0ó­SÌ'ed=lAÙ+"\`Æjƒ½Z´òâãÇäù)š'†šë¶-?¼ôû)M)¨MÉ:ÕâœåÙCìþZ¤Ds—†['õ…Ól•§¡ qœDgqA0²"q8$#{ÿ©¾ª¢õJß­Þ轟üÔý'¼'­£³ôƞÙÌmÿ{™kÎȄ㎶lg£¬ô\2ê¥ãx¥Ç&ëJe9ð0¿y#Mƒ

==> preamble/.git/objects/ee/727f75b804f285bb39d7d291eaa975e811c71d <==
x­V]kä6í³ŅÁ°»
CfºK—@ Ð(´°ì¶û2žÙ¾¶ÕȒ'ä$SãþöI3O²K_ú'xt¯äsÏ=÷È¥2%m¿{ÿö›bt<ˆêN´<UÒóœe¹¨ï…®¸&ر÷R·Ù2±—•5!²éÏOÔ†ŽµðÒèeâNôle%ô~*EÉ
éÈçGÏÚ!ÕQc,yQ*vËm"°V拥~T^Zóp¹Zs‡ýîrµw\±R3åR{kê±bG…ïXÔ$tMÅ)p*Ó£~Oƒ°¢µbèÈK¯8+4? Ö#*úÃ9<ï6û©ð(¢l¦'û¡›V›y^ÏY~±Åå³=§\¤fù`ͽ¬™ÌHKLTÐ-¸&Dá¿ÔÄz‡'Y<߃ݳöàK6•Ó ˜T VêËë:­f…b_,C–•x̊F.yÝI­¼ŸÂ{Ðþ~Íjh"ÞÑ+<V"b%˃Ñ–md4=Ž–¯¨}–÷²í<iã©dŠ{‰6Ӄô9ԕα{½D3¥c†_µ¤…ËýøùÃG6¼Ö£1GêÎ͑<OrͅÑ\),;Çí<ñº}
>ßÍ^(¤x꜔åP=õÆ2Šk€Q¡IÞ
èɑÑ-Q¢&+[™Q{¶"7x,ÙÎÓ@'Òxoú¯½ˆSì-6Z^րSB(ót½~ÿîEF:ý?''f—)›—çĒxÁ2ïûЏß1Sèô…c3Ah¨ý[ÛZvNÞ3¥Zb'¢ÔIÍ<ï¶ûÝ>›Š'¡ø¨¾ r¬GÉÞ¾Zmd)«7¯¯7¾‰·×ë­ÔWA¨IðXؼÃÊj³Ÿqä¿8k‰û« ©fWY™¤­¤ó/Q/2žá^4­¶sž¦®øŠð—­Œ#ÙÁCRZèŠSÓ
&róÏ|*bq0ªÈ(ÿ#Î(e¢A0d4xð6:išåe‹\EÊz³;"K4O@é:1ð™l ÈòŸ¸)P/`óä
Ðü³›QðQ p™qpxa[P3*E'Í¢Ç
8iÇåLžOrAA!{žŽÔUfx²ÚâœøŒÇ§@4ã‹MÉõŒV`Hnáê€ Ë?¤k.yÂõÁcKóxyíb¼gߙúÖË»¿÷S_ǵ:ÐC¹aô5x ìéxŒóáz1
9Ž£J¸ÛÂ(‡!¡9RsSû®c'V›Õö8­5㐭¶9þ!ï‡j´xŸ©Ihˆ¸.à)Ç×%¯wQ˜'tÈ
>…²WšûdÕT›hÓR;¶þIS±ªƒ_Æ||ÿ ÿ¿ 1¶b|5"[ZÂä§ëT‹…*£ý5:/|r¤O'¥‹BL£vwb+ÊÈO'~55R©»½<˜¶à˜ڝçô›©"¢ÏÂÊø±r{Só
&ý¿ÖõMö/cp

==> preamble/.git/objects/fd/d5555aea64227f4067c24280cdc299115ed3af <==
x•ÎK
Â0€a×9Å\@™É£iAĸ/ÇDmSâäþŠ7póï>øS]×Y@ksÆäâTl˜ØyË%tv2ì3»8a¦â¤Õo9Z4ã˜m6!Eím*¾PˆÞ'³š3s"?ªÐåUÜkä&­np–o¯±Ÿ8÷ÐàÈèˆàˆQ¥ß›ðJÝjcXkîKhðޗYdޞê( G

==> preamble/common.tex <==
\input{preamble/commonNoTikz}
\input{preamble/graphicsTikz}
\input{preamble/robotics}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/commonNoTikz.tex <==
\input{preamble/fixes}
%Note: pagination needs to be loaded after graphics, because mdframed
%needs to be loaded after xcolor to keeep the our options for the latter
\input{preamble/graphics}
\input{preamble/pagination}
%
\input{preamble/utilities}
\input{preamble/math}
\input{preamble/operators}
\input{preamble/graphTheory}
\input{preamble/notation}
\input{preamble/units}
\input{preamble/markupAndCommenting}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}


==> preamble/courseExam.tex <==
\usepgflibrary{shapes.arrows}

\input{preamble/courseFormatting}
\usepackage{probsoln}
\tikzset{ax/.style={very thick,-latex},pnt/.style={minimum size=5pt,fill=blue,circle,inner sep=0pt}}

%ref: https://tex.stackexchange.com/questions/201197/latex-using-the-matching-environment-in-the-exam-documentclass
\usepackage{multicol}

\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\fullwidth{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}
\newcommand{\vspacefivelines}{\vspacebox{6}}
\newcommand{\vspacesixlines}{\vspacebox{7}}
\newcommand{\vspacesevenlines}{\vspacebox{8}}

%% Create a Matching question format
\newcommand*\Matching[1]{
\ifprintanswers
    \textbf{#1}
\else
    \rule{2.7in}{0.5pt}
\fi
}
\newlength\matchlena
\newlength\matchlenb
\settowidth\matchlena{\rule{2.7in}{0pt}}
\newcommand\MatchQuestion[2]{%
    \setlength\matchlenb{\linewidth}
    \addtolength\matchlenb{-\matchlena}
    \parbox[t]{\matchlena}{\Matching{#1}}\enspace\parbox[t]{\matchlenb}{#2}}


==> preamble/courseFormatting.tex <==
% Make font for captions smaller (saves space and visually separates them from the main text)
\usepackage[font={footnotesize,sf}]{caption}

% Print menu and key command descriptions
% \usepackage{menukeys}

% make underscore work without escaping in text mode
\usepackage{underscore}

% Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue3}\sffamily}

% Perfect 1-inch margins
\usepackage[margin=1in]{geometry}
\usepackage[medium,compact]{titlesec}
\usepackage{longtable}
\titleformat*{\section}{\titlestyle \Large}
\titleformat*{\subsection}{\titlestyle \large \itshape}

% Lists (requires enumitem package):
% Font for description
\setlist[description]{font=\color{DodgerBlue3}}
% Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

% Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}

% Displayed quotations (used to define an environment for function specification)
\usepackage{csquotes}

% Include code
\input{preamble/formattingCode}

% formatting for the description of a function's input/output arguments
\mdfdefinestyle{functionspecification}{%
  linecolor=DodgerBlue3,
  rightline=false, topline=false, bottomline=false,
  outerlinewidth=1.35,
  roundcorner=10pt,
  innerleftmargin=1.2em,
  innertopmargin=0.3em,
  innerbottommargin=0.3em,
  leftmargin=1pt,
  skipabove=0.5em,
  skipbelow=0.5em,
  backgroundcolor=white}

\newcommand{\dstar}{$\bigstar$}

% Clever cross-references
\usepackage{cleveref}


==> preamble/courseLanguage.tex <==
\newif\ifmatlab
\matlabtrue
% Enable conditional part based on whether the language used is Matlab or not
% \ifmatlab
% % use Matlab
% \else
% % use Python or something else
% \fi

\newcommand{\hwlanguage}{\ifmatlab{}Matlab\else{}Python\fi{}}
\newcommand{\ifmtlb}[2]{\ifmatlab{}#1\else{}#2\fi{}}
\newcommand{\vartrue}{\var{\ifmatlab{}true\else{}True\fi{}}}
\newcommand{\varfalse}{\var{\ifmatlab{}false\else{}False\fi{}}}
\newcommand{\varlang}[2]{\var{\ifmtlb{#1}{#2}}}

\newcommand{\langfield}[1]{\ifmtlb{.#1}{['#1']}}
\newcommand{\functionlanguage}[3]{\function{\ifmatlab{}#1\else{}#2\fi{}}{#3}}
\newcommand{\functionheaderlanguage}[4][]{%
  \ifmatlab{}%
  \functionheader[#1]{#2}{#4}%
  \else{}%
  \fname[Method]{#3}%
  \fi{}%
}
\newenvironment{functionspeclang}[1]
{\functionspecification\ifmatlab{}\else{}\ffilename{#1}\fi{}}
{\endfunctionspecification}

\NewEnviron{functionclassspeclang}[3][]{%
  \ifmatlab{}%
  \begin{functionspecification}
    \BODY%
  \end{functionspecification}
  \else{}%
  \begin{classspecification}%
    \cname{#2}%
    \ffilename{#3}%
    \ifnotempty{#1}{
      \begin{cdescription}
        #1
      \end{cdescription}
    }
    \begin{functionspecification}
      \BODY%
    \end{functionspecification}
  \end{classspecification}%
  \fi{}%
}

==> preamble/courseProblemSet.tex <==
\input{preamble/courseFormatting}
\input{preamble/courseLanguage}
\newcommand{\hwtitle}[2]{
\ifmatlab
\title{Homework #2 (Matlab version)}
\else
\title{Homework #2 (Python version)}
\fi
\author{#1 - Prof. Tron}
\date{\today}
\edef\hwnumber{#2}
}


%Facilities for markers file
% open file the beginning of the document
\AtBeginDocument{%
\newwrite\markerstream
\immediate\openout\markerstream=\jobname.mlg
}
% close the file at the end of the document
\AtEndDocument{%
\immediate\closeout\markerstream
}
%definition similar to \typeout, but for markers
\makeatletter
\newcommand{\markerout}[1]{\begingroup \set@display@protect \immediate \write \markerstream {#1}\endgroup}
\makeatother

\usetikzlibrary{intersections}

\titleformat{\section}{\titlestyle\large\bfseries}{Problem \thesection:}{0.5ex}{}
%\titleformat{\subsection}{\normalfont\bfseries}{Problem \thesubsection:}{0.5ex}{}
\titleformat{\paragraph}[runin]{\titlestyle\normalsize\bfseries}{}{2pt}{}

%Macro for paragraph header for preparation steps to questions
%\newcommand{\preparation}{\smallskip\par\noindent\textbf{\titlestyle Preparation.~}}

\newcommand{\preparation}[1][]{%
\smallskip\par\noindent%
\textbf{\titlestyle Preparation\displayifnotempty{~(}{#1}{)}.~}}

%New custom counter for question
\newcounter{question}[section]

%Macro for writing points for the current question to the log file.
\newcommand{\pointmarker}{\typeout{Question points marker [\thesection.\thequestion] [\questionpoints]}}

\makeatletter
%Makes questions that:
%- are automatically numbered using the format <sectionNumber>.<questionNumber>
%- can be referred to using the usual \label-\ref mechanism
%- if the optional argument is not empty, this is displayed in parenthesis (typically, this will be a \points{n} or a \optional command). If the optional argument is empty, a single point is silently added to the point counter.
\newcommand{\question}[1][]{%
\smallskip\par\noindent%
\refstepcounter{question}\zerovar{\questionpoints}%
\sbox\boxifnotempty{\textbf{\titlestyle #1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
\textbf{\titlestyle Question \thesection.\thequestion\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
\ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
\def\@currentlabel{{\thesection.\thequestion}}\pointmarker%
\markerout{Marker question [nolabel] [\thesection.\thequestion]}}%

%Commands that defines a new `labeled' question, which uses a separate counter but the same total point count. A new label with the same name must be defined separately
\newcommand{\newquestionlabel}[1]{%
\newcounter{question#1}[section]%
\expandafter\newcommand\csname question#1\endcsname[1][]{%
\smallskip\par\noindent%
\refstepcounter{question#1}\zerovar{\questionpoints}%
\sbox\boxifnotempty{\textbf{\titlestyle ##1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
\textbf{\titlestyle Question \csname #1\endcsname~\thesection.\csname thequestion#1\endcsname\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
\ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
\def\@currentlabel{{#1~\thesection.\csname thequestion#1\endcsname}}\pointmarker%
\markerout{Marker question [#1] [\thesection.\csname thequestion#1\endcsname]}}%
}
\makeatother

\newquestionlabel{code}
\newquestionlabel{report}
\newquestionlabel{optional}
\newquestionlabel{provided}
\newquestionlabel{image}
\newquestionlabel{video}
\newquestionlabel{scan}
\newquestionlabel{feedback}

\newcommand{\hintquestion}[1]{\paragraph{Hint
for question \ref{#1}:~}}
\newcommand{\hint}{\paragraph{Hint:~}}

\newcommand{\answer}[1][]{\smallskip\leavevmode\\\noindent\textbf{Answer \thesection.\thequestion#1:~}}

\newcommand{\updated}[1]{{\color{red} #1}}

\newcolorlabel{labeloptional}{DodgerBlue3}
\newcommand{\optional}{\labeloptional{optional}}
\newcolorlabel{labelprovided}{Orange1}
\newcommand{\provided}{\labelprovided{provided}}
\newcolorlabel{labelvideo}{Coral2}
\newcommand{\video}{\labelvideo{video}}
\newcolorlabel{labelimage}{DarkOrchid2}
\newcommand{\image}{\labelimage{image}}
\newcolorlabel{labelcode}{SlateBlue2}
\newcommand{\code}{\labelcode{code}}
\newcolorlabel{labelscan}{Chocolate3}
\newcommand{\scan}{\labelcode{scan}}
\newcolorlabel{labelnew}{OliveDrab3}
\newcommand{\lbnew}{\labelnew{new}}
\newcolorlabel{labelreport}{OliveDrab3}
\newcommand{\report}{\labelreport{report}}
\newcolorlabel{labelgoal}{Black}
\newcommand{\goal}{\labelgoal{Goal}}
\newcolorlabel{labelfeedback}{SeaGreen4}
\newcommand{\feedback}{\labelfeedback{feedback}}

%Camera icon
\usepackage{fontawesome}
\newcommand{\screenshot}{\textcolor{DarkOrchid2}{\faCamera~Take a screenshot.}}

\tikzset{point/.style={inner sep=0pt,fill=black,circle,minimum size=4pt}}

%macros for keeping track of points (total, and for current question)
\zerovar{\totalpoints}
\zerovar{\bonuspoints}
\zerovar{\questionpoints}
\newcommand{\increasepoints}[1]{\addtovar{\totalpoints}{#1}\addtovar{\questionpoints}{#1}}
\newcommand{\points}[1]{#1 point\ifthenelse{\equal{#1}{1}}{}{s}\increasepoints{#1}}
\makeatletter
\newcommand{\totalpointswithbonus}[1]{\pgfmathparse{\storeddef{totalpoints}+#1}\pgfmathresult\typeout{Total points marker [\pgfmathresult]}}
\makeatother

\newstoreddef{totalpoints} %remember total number of points in aux file

% answer boxes
\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\par\bigskip{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}
\newcommand{\vspacefivelines}{\vspacebox{6}}
\newcommand{\vspacesixlines}{\vspacebox{7}}

% text fields
\newcommand{\textrowfield}[1]{\par\noindent#1: \enspace\hrulefill}

% formatting for the description of a function's input/output arguments
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,
skipbelow=0.5em,
backgroundcolor=white}
\mdfdefinestyle{classspecification}{%
linecolor=DarkOliveGreen3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,
skipbelow=0.5em,
backgroundcolor=white}
%Note: I was not able to avoid duplication of options.

\newenvironment{functionspecification}{\markerout{Marker function [start]}\begin{mdframed}[style=functionspecification]}
{\markerout{Marker function [end]}\end{mdframed}}%
\newenvironment{classspecification}{\markerout{Marker class [start]}\begin{mdframed}[style=classspecification]}
{\markerout{Marker class [end]}\end{mdframed}}%
%\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\newenvironment{cdescription}{\fdescription}{\endfdescription}
\NewEnviron{frequirements}{\par\noindent{\titlestyle Requirements}: \BODY\markerout{Marker text [requirements] [start]^^J\BODY^^JMarker text [requirements] [end]}\par}
\newcommand{\cname}[1]{\noindent{\titlestyle Class name}: \var{#1}\par}
\newenvironment{finputs}{\markerout{Marker argument_group [start] [inputs]}\noindent{\titlestyle Input arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foptional}{\markerout{Marker argument_group [start] [optional]}\noindent{\titlestyle Optional arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foutputs}[1][Output]{\markerout{Marker argument_group [start] [outputs]}\noindent{\titlestyle #1 arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newcommand{\freturns}[2][]{\noindent{\titlestyle Returns}: \var{#2}\displayifnotempty{ (type }{\var{#1}}{)}}
\newcommand{\argument}[4][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2}
\ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [#4]}dim. \vardim{#3}{#4}\ifnotempty{#1}{, }}%
\ifnotempty{#1}{\markerout{Marker argument [type] [#1]}type \var{#1}\markerout{Marker argument [end]}}
)}\markerout{Marker argument [end]}}%removed the \var{}
\newcommand{\argumentlist}[3][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2} %
\ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [1]} length #3\ifnotempty{#1}{, }}%
\displayifnotempty{\markerout{Marker argument [type] [#1]}type }{\var{#1}}{})}\markerout{Marker argument [end]}}
\newcommand{\argumentscalar}[2][]{\argument[#1]{#2}{}{}}
\newcommand{\fheader}[3][]{\noindent{\titlestyle Header}: \function[#1]{#2}{#3}\par}
\newcommand{\fname}[2][Function]{\noindent{\titlestyle #1 name}: \var{#2}\par}
\newcommand{\ffilename}[1]{\noindent{\titlestyle File name}: \file{#1}\par}
\newcommand{\functionheader}[3][]{\markerout{Marker function_header [#1] [#2] [#3]}\function[#1]{#2}{#3}\par}

% Commands to indicate functions and files that are provided but not fully specified
\newcommand{\mfunctionprovided}[3][]{\markerout{Marker file_provided [#2.m]}\function[#1]{#2}{#3}}
\newcommand{\fileprovided}[2][]{\markerout{Marker file_provided [#1#2]}\file{#2}}
\newcommand{\fileincluded}[2][]{\markerout{Marker file_provided [#1#2]}}
%note: fileprovided and fileincluded differ on whether the file name is inserted in the TeX output (in both cases, it is inserted in the marker log)

%ROS node specification
\newenvironment{nodespecification}{\begin{mdframed}[style=functionspecification]%
\newcommand{\filename}[1]{\par{\titlestyle File name:} \file{##1}}
\renewenvironment{description}{\par\noindent{\titlestyle Description:}}{\par}%
\newenvironment{subscribers}{\par\noindent{\titlestyle Subscribes to topics:}}{}%
\newenvironment{publishers}{\par\noindent{\titlestyle Publishes to topics:}}{}%
%
}{\end{mdframed}}

\newcommand{\rostopic}[2]{\var{#1} (type \var{#2})}

% Macros for questions where student need to draw on axes
\newcommand{\drawingaxes}[1][]{\draw[gray] (-5,-5) grid (5,5);
\draw[very thick, -latex] (-5.7,0) -- (5.7,0) coordinate (a1);
\draw[very thick, -latex] (0,-5.7) -- (0,5.7) coordinate (a2); #1}

\newcommand{\shifteddrawingaxes}[1][]{
\begin{scope}[xshift=18cm]
\drawingaxes[#1]
\end{scope}
}

\newcommand{\drawexercise}[2][]{\begin{center}
\begin{tikzpicture}[scale=0.6]
\node[text width=7cm,anchor=west]{#2};
\shifteddrawingaxes[{\node at ($(a1)-(0,1.2em)$) {$x_1$}; \node at ($(a2)+(1.2em,0)$) {$x_2$}; #1}]
\end{tikzpicture}
\end{center}
}

\input{preamble/courseProblemSetQuotes}

==> preamble/courseProblemSetQuotes.tex <==
% Insert a random quote from file
% ref: https://tex.stackexchange.com/questions/187000/can-latex-select-a-random-line-from-another-file
\usepackage{datatool}
\newcommand{\quotecomma}{,{}}
\newcommand{\randomquote}[1][preamble/quotes.txt]{%
  \DTLsetseparator{|}%
  \DTLloadrawdb[keys={Number,Quote,Author}]{quotes}{#1}% Load quotes
  \edef\RandomQuote{\number\numexpr1+\pdfuniformdeviate\DTLrowcount{quotes}}% Identify random quote
  \dtlgetrow{quotes}{\RandomQuote}% Retrieve random quote
  \dtlgetentryfromcurrentrow{\Quote}{1}\dtlgetentryfromcurrentrow{\Author}{2}%
  ``\Quote''\\---~\emph{\Author}%
}
\newcommand{\randomquotebox}{
  \begin{mdframed}
    \randomquote{}
  \end{mdframed}
}

\newcommand{\copyrightnote}{\copyright\the\year Boston University and Roberto Tron. All rights reserved. No distribution without written permission.}


==> preamble/courseProblemSetSectionsLettered.tex <==
%Change format of numbering for questions to letters instead of numbering
\renewcommand{\thequestion}{\alph{question}}


==> preamble/courseSyllabus.tex <==
\input{preamble/courseFormatting}
\usepackage{etoolbox}

\newlength{\topicwidth}
\newlength{\topicdatewidth}
\setlength{\topicdatewidth}{19mm}
\newlength{\duewidth}
\setlength{\duewidth}{23mm}

%Create a topictable environment from the longtable environment
\newenvironment{topictable}[1][2cm]%
{\newcommand{\picswidth}{#1}\setlength{\topicwidth}{\textwidth-\picswidth-\topicdatewidth-\duewidth-12.5mm}%
\setcounter{topic}{1}\begin{longtable}{p{\picswidth}p{\topicwidth}p{\topicdatewidth}p{\duewidth}}}%
{\end{longtable}}

%Prepare counter and relative macros for handling array of class dates
\newcount\i
\pgfmathsetcount{\i}{0}
\def\classdate{\pgfprint{\classdatearray[\i]}\global\advance\i 1\relax}

% Counters for topic and subtopic
\newcounter{topic}
\newcounter{subtopic}

% Toggle for controlling pod switching
\newtoggle{pod}
\toggletrue{pod}
\newcommand{\podtoggle}{\iftoggle{pod}{\pods{A,B}\global\togglefalse{pod}}{\pods{C,D}\global\toggletrue{pod}}}

% Labels
\newcolorlabel{labelhw}{Orange1}
\newcommand{\hwrel}[1]{\par\labelhw{HW #1 Rel}~}
\newcommand{\hwdue}[1]{\labelhw{HW #1}}
\newcolorlabel{paperdue}{Tomato1}
\newcolorlabel{examdue}{Tomato1}
\newcolorlabel{labelMH}{DodgerBlue3}
\newcommand{\mhday}{\labelMH{M-H}~}
\newcolorlabel{labelqz}{Sienna3}
\newcommand{\qzdue}[1]{\labelqz{QZ #1}~}
\newcolorlabel{labelactivity}{Snow4}
\newcommand{\activity}{\labelactivity{Activity}~}
\newcommand{\readinggroup}{\labelqz{Reading group}~}
\newcolorlabel{labelpod}{DarkOliveGreen3}
\newcommand{\pods}[1]{\labelpod{Pods #1}~}
\newcommenter{instructor}{DarkOliveGreen3}



% Topichead
\def\topichead#1#2#3{\rowcolor{SlateGray1}{\setcounter{subtopic}{1}\rule{0pt}{16pt}\titlestyle Topic \arabic{topic}\addtocounter{topic}{1}} & \multicolumn{3}{l}{{\titlestyle #1:} #2 \rule[-8pt]{0pt}{12pt}}\\\tikz[overlay]{\node[anchor=north west,inner sep=0pt]{\includegraphics[width=\picswidth,keepaspectratio]{figures/#3}};}}
\def\firstsubtopic#1{ & \makecell[{{p{\topicwidth}}}]{\rule{0pt}{14pt}#1}\addtocounter{subtopic}{1}}
\makeatletter
\def\subtopic{\@ifstar\@subtopicstar\@subtopic}
\def\@subtopic#1{\\ \cmidrule{2-4} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
\def\@subtopicstar#1{\\ \cmidrule{2-2} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
\makeatother
\def\activitytopic#1{\\ \cmidrule{2-4} & \multicolumn{3}{l}{\cellcolor{Snow2}{\parbox{\topicwidth+\topicdatewidth+\duewidth}{\activity #1}}}}
% \def\topicdate#1{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\makeatletter
\def\topicdate{\@ifstar\@topicdatestar\@topicdate}
\newcommand{\@topicdate}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\newcommand{\@topicdatestar}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}% Add \podtoggle for LfA
\makeatother
\def\due#1{& \makecell[{{p{\duewidth}}}]{#1}}
\def\endtopic{\\}
% TODO: Add automatic test to check if a subtopic is the first subtopic, and adjust the formatting accordingly.
% The subtopic counter is already there, but due to conflicts with the tabular environment, I was not able to include the test inside the \subtopic macro.
% \def\tpctest{\noalign{\ifnum\value{subtopic}=1{}\else{\hrule}\fi}}


==> preamble/fixes.tex <==
%fixes to the latex2e kernel
%\usepackage{fixltx2e} %this is not needed after 2015
\usepackage{fix-cm}
\usepackage{etex}

%fix double floats numbering and positioning
\usepackage{dblfloatfix}

%checks for obsolete packages
\usepackage{nag}


%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/formattingCode.tex <==
% Include code and org files
\usepackage{listings}
% Smaller fixed-width font, automatic breaking of long lines, ignore indentation in list environments
\lstset{basicstyle=\footnotesize\ttfamily,breaklines=true,resetmargins=true}


==> preamble/generateGraphLocalization <==
#!/usr/bin/env python
# Note: in the list of node and edge quantities: first element is the name to use in the command name,
# the second is the one to use in the definition

import os
f=open('graphLocalization.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Notation for nodes\n')
nodeIndexList=['i','j']
nodeStateDoubleList=[['R','R'],['T','T']]
for index in nodeIndexList:
    for state in nodeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
        f.write('\\newcommand{\\d'+state[0]+index+'}{\\dot{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dd'+state[0]+index+'}{\\ddot{'+state[1]+'}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

edgeIndexList=['ij','ji']
edgeStateDoubleList=[['R','R'],['T','T'],['beta','\\beta'],['c','c'],['d','d'],['q','q'],['l','\\lambda'],['varphi','\\varphi'],['g','g']]

f.write('% Notation for edges\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Notation for edges, measured quantities\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\t'+state[0]+index+'}{\\tilde{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dt'+state[0]+index+'}{\\dot{\\tilde{'+state[1]+'}}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Node state differences\n')
f.write('\\newcommand{\\xjmi}{x_j-x_i}\n')
f.write('\\newcommand{\\vjmi}{v_j-v_i}\n')
f.write('\\newcommand{\\nxjmi}{\\norm{\\xjmi}}\n')
f.write('\n')

f.write('% Notation for desired quantities\n')
quantityTripleList=[['x','x','i'],['x','x','j'],['beta','\\beta','ij'],['d','d','ij']]
for quantity in quantityTripleList:
    f.write('\\newcommand{\\'+quantity[0]+'g'+quantity[2]+'}{'+quantity[1]+'_{g,'+quantity[2]+'}}\n')

f.close()






        


==> preamble/generateNotation <==
#!/usr/bin/env python
import string
import os
f=open('notation.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Shortand notation for vectors and their derivatives\n')
for c in string.ascii_lowercase+string.ascii_uppercase:
    f.write('\\providecommand{\\v'+c+'}{\\vct{'+c+'}}\n')
    f.write('\\providecommand{\\dv'+c+'}{\\dot{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\tv'+c+'}{\\tilde{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\dtv'+c+'}{\\dot{\\tilde{\\vct{'+c+'}}}}\n')
f.write('\n')
for c in [['beta','\\beta'],['sigma','\\sigma']]:
    f.write('\\providecommand{\\v'+c[0]+'}{\\boldsymbol{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dv'+c[0]+'}{\\dot{\\boldsymbol{'+c[1]+'}}}\n')
f.write('\n')
for c in ['e']:
    f.write('\\providecommand{\\t'+c+'}{\\tilde{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for derivatives and bold of symbols\n')
for s in ['gamma', 'Delta', 'pi', 'varphi']:
    c = [s, '\\'+s]
    f.write('\\providecommand{\\d'+c[0]+'}{\\dot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dd'+c[0]+'}{\\ddot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\v'+c[0]+'}{\\bm{'+c[1]+'}}\n')
f.write('\n')


f.write('% Shortand notation for matrices\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\m'+c+'}{\\vct{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for calligraphic upper case letters\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\c'+c+'}{\\mathcal{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for some tilded symbols and their derivatives\n')
symbolDoubleList=[['x','x'],['y','y'],['varphi','\\varphi']]
for symbol in symbolDoubleList:
    f.write('\\providecommand{\\t'+symbol[0]+'}{\\tilde{'+symbol[1]+'}}\n')
    f.write('\\providecommand{\\dt'+symbol[0]+'}{\\dot{\\tilde{'+symbol[1]+'}}}\n')
f.write('\n')

f.close()


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphTheory.tex <==
%memberships
\newcommand{\iV}[1][]{{i \in V_{#1}}}
\newcommand{\ijE}[1][]{(i,j) \in E_{#1}}

%operators
\DeclareMathOperator{\dg}{{deg}}
\DeclareMathOperator{\diam}{{Diam}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/graphics.tex <==
%colors
\makeatletter
\@ifpackageloaded{xcolor}{}{%
\usepackage[table,x11names,dvipsnames,svgnames]{xcolor}%
}
\makeatother

%colors in table
\usepackage{colortbl}

%pdf
\usepackage{graphicx}
\usepackage{wrapfig}

% Lyft colors (see https://design.lyft.com/re-approaching-color-9e604ba22c88)
\input{preamble/graphicsColors}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/graphicsColors.tex <==
\definecolorset{RGB}{lyft}{}{Red,194,39,36;Sunset,202,53,33;Orange,205,68,20;Amber,200,117,42;Yellow,242,169,52;Citron,186,188,44;Lime,112,159,33;Green,56,139,31;Mint,45,118,56;Teal,52,133,135;Cyan,60,132,202;Blue,55,94,248;Indigo,64,13,247;Purple,115,42,248;Pink,176,25,145;Rose,176,32,75}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}
\usepackage{cprotect}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
  \begin{tikzpicture}[scale=0.7]%
    \input{#1/sketch/#2}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[2][.]{\section{$\mathrm{#2}$}%
\tikzsetnextfilename{#2}%
\input{#1/tikz/#2}%
\endpgfgraphicnamed%
}

%command to insert an equation and externalize
\newcommand{\insertequationframe}[2]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
\begin{tikzpicture}
  \node{$\begin{aligned}
          #2  
        \end{aligned}$};
\end{tikzpicture}
\endpgfgraphicnamed%
}


==> preamble/graphicsTikz.tex <==
%TikZ and common libraries
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}
\usetikzlibrary{chains,scopes}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{backgrounds}

%Example figure
\newcommand{\picplaceholder}[1]{\tikz{\draw (-2,-1.5) rectangle (2,1.5); \node[font=\tiny] {#1};}}

%Draw normalized vector between two coordinates
\newcommand\normalize[2][(0,0)]{%
  \draw[blue,->] (#1) -- ($(#1)!1cm!(#2)$) coordinate (#1#2norm)}

%Quotatures
\tikzset{
  dim above/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let
        \p1=($(\tikztostart)!1.5em!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!1.5em!-90:(\tikztostart)$)
        in(\p1) -- (\p2) node[pos=.5,sloped,above]{#1};
        \endpgfinterruptpath
      }
    }
  },
  dim double above/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let
        \p1=($(\tikztostart)!3em!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!3em!-90:(\tikztostart)$)
        in(\p1) -- (\p2) node[pos=.5,sloped,above]{#1};
        \endpgfinterruptpath
      }
    }
  },
  dim below/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let 
        \p1=($(\tikztostart)!-1em!-90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!-1em!90:(\tikztostart)$)
        in (\p1) -- (\p2) node[pos=.5,sloped,below]{#1};
        \endpgfinterruptpath
      }
    }
  },
}

%Right angle symbol
\tikzset{
    right angle quadrant/.code={
        \pgfmathsetmacro\quadranta{{1,1,-1,-1}[#1-1]}     % Arrays for selecting quadrant
        \pgfmathsetmacro\quadrantb{{1,-1,-1,1}[#1-1]}},
    right angle quadrant=1, % Make sure it is set, even if not called explicitly
    right angle length/.code={\def\rightanglelength{#1}},   % Length of symbol
    right angle length=2ex, % Make sure it is set...
    right angle symbol/.style n args={3}{
        insert path={
            let \p0 = ($(#1)!(#3)!(#2)$) in     % Intersection
                let \p1 = ($(\p0)!\quadranta*\rightanglelength!(#3)$), % Point on base line
                \p2 = ($(\p0)!\quadrantb*\rightanglelength!(#2)$) in % Point on perpendicular line
                let \p3 = ($(\p1)+(\p2)-(\p0)$) in  % Corner point of symbol
            (\p1) -- (\p3) -- (\p2)
        }
    }
}

%Horizontally fit an image between two coordinates
\newcommand{\imageBetween}[3]{\draw (#2) let \p1 = ($ (#3) - (#2) $) in node[inner sep=0pt,anchor=south west, text width={veclen(\x1,\y1)}] {\includegraphics[width=\linewidth]{#1}};}

%Get angle between a line going through two points and the horizontal
%direction
\newcommand{\pgfextractangle}[3]{%
    \pgfmathanglebetweenpoints{\pgfpointanchor{#2}{center}}
                              {\pgfpointanchor{#3}{center}}
    \global\let#1\pgfmathresult  
}

%Arrow to be used to indicate something in the text
\usetikzlibrary{shapes.arrows}
\newcommand{\commentarrow}[1][Azure4]{\tikz[baseline=-3pt]{\node[shape border uses incircle, fill=#1,rotate=180,single arrow, inner sep=1pt, minimum size=6pt, single arrow head extend=2pt]{};}}

%Draw a test grid to help with positioning
\newcommand{\tikztestgrid}[3][cm]{
  \coordinate (testgrid origin) at (0,0);
  \coordinate (testgrid bl) at (-#2#1/2,-#3#1/2);
  \coordinate (testgrid ur) at (#2#1/2,#3#1/2);
  \begin{scope}[opacity=0.5]
    \draw[cyan!50] (testgrid bl) grid[step=0.1#1] (testgrid ur);
    \draw[cyan] (testgrid bl) grid[step=1#1] (testgrid ur);
  \end{scope}
  \draw[red,-latex] (testgrid bl|-testgrid origin) -- (testgrid ur|-testgrid origin);
  \draw[red,-latex] (testgrid bl-|testgrid origin) -- (testgrid ur-|testgrid origin);
  \node[circle,fill=black,minimum size=3pt,inner sep=0pt] at (testgrid origin) {};
}


==> preamble/letter.tex <==
\usepackage{graphicx}
\usepackage[table,x11names,dvipsnames,svgnames]{xcolor}%
\usepackage{pgffor}
\input{preamble/markupAndCommenting}
\input{preamble/splitting}
\input{preamble/utilities}
\usepackage{hyperref}
\pagestyle{empty}

\KOMAoptions{fromphone,fromemail,fromlogo,backaddress=false,foldmarks=false}
\setkomavar{fromname}{Assistant Professor Roberto Tron}
\setkomavar{fromaddress}{Mechanical Engineering, System Engineering\\110 Cummington Mall, Room 301\\Boston, MA 02215}
\setkomavar{fromphone}{+1 617~353~3951}
\setkomavar{fromemail}{tron@bu.edu}
\setkomavar{fromlogo}{\includegraphics[height=5.8em]{figures/BostonUniversity}}
\setkomafont{fromname}{\sffamily\footnotesize}
\setkomafont{fromaddress}{\sffamily\footnotesize}
\setkomavar{signature}{\includegraphics[width=5cm]{figures/signature}\\Roberto Tron}

\newcommand{\noaddress}{
  \csname @setplength\endcsname{sigbeforevskip}{\parskip}
  \csname @setplength\endcsname{refvpos}{\useplength{toaddrvpos}}
}


==> preamble/math.tex <==
% AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother
% Generic symbols (e.g., \degree)
\usepackage{gensymb}
% Prescripts, squashed summations, and others
\usepackage{mathtools}
% Bold greek letters
\usepackage{bm}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
%\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables:
%%% mode: latex
%%% End:


==> preamble/notation.tex <==
% This file was generated by the scriptgenerateNotation
% Do not modify this file directly

% Shortand notation for vectors and their derivatives
\providecommand{\va}{\vct{a}}
\providecommand{\dva}{\dot{\vct{a}}}
\providecommand{\tva}{\tilde{\vct{a}}}
\providecommand{\dtva}{\dot{\tilde{\vct{a}}}}
\providecommand{\vb}{\vct{b}}
\providecommand{\dvb}{\dot{\vct{b}}}
\providecommand{\tvb}{\tilde{\vct{b}}}
\providecommand{\dtvb}{\dot{\tilde{\vct{b}}}}
\providecommand{\vc}{\vct{c}}
\providecommand{\dvc}{\dot{\vct{c}}}
\providecommand{\tvc}{\tilde{\vct{c}}}
\providecommand{\dtvc}{\dot{\tilde{\vct{c}}}}
\providecommand{\vd}{\vct{d}}
\providecommand{\dvd}{\dot{\vct{d}}}
\providecommand{\tvd}{\tilde{\vct{d}}}
\providecommand{\dtvd}{\dot{\tilde{\vct{d}}}}
\providecommand{\ve}{\vct{e}}
\providecommand{\dve}{\dot{\vct{e}}}
\providecommand{\tve}{\tilde{\vct{e}}}
\providecommand{\dtve}{\dot{\tilde{\vct{e}}}}
\providecommand{\vf}{\vct{f}}
\providecommand{\dvf}{\dot{\vct{f}}}
\providecommand{\tvf}{\tilde{\vct{f}}}
\providecommand{\dtvf}{\dot{\tilde{\vct{f}}}}
\providecommand{\vg}{\vct{g}}
\providecommand{\dvg}{\dot{\vct{g}}}
\providecommand{\tvg}{\tilde{\vct{g}}}
\providecommand{\dtvg}{\dot{\tilde{\vct{g}}}}
\providecommand{\vh}{\vct{h}}
\providecommand{\dvh}{\dot{\vct{h}}}
\providecommand{\tvh}{\tilde{\vct{h}}}
\providecommand{\dtvh}{\dot{\tilde{\vct{h}}}}
\providecommand{\vi}{\vct{i}}
\providecommand{\dvi}{\dot{\vct{i}}}
\providecommand{\tvi}{\tilde{\vct{i}}}
\providecommand{\dtvi}{\dot{\tilde{\vct{i}}}}
\providecommand{\vj}{\vct{j}}
\providecommand{\dvj}{\dot{\vct{j}}}
\providecommand{\tvj}{\tilde{\vct{j}}}
\providecommand{\dtvj}{\dot{\tilde{\vct{j}}}}
\providecommand{\vk}{\vct{k}}
\providecommand{\dvk}{\dot{\vct{k}}}
\providecommand{\tvk}{\tilde{\vct{k}}}
\providecommand{\dtvk}{\dot{\tilde{\vct{k}}}}
\providecommand{\vl}{\vct{l}}
\providecommand{\dvl}{\dot{\vct{l}}}
\providecommand{\tvl}{\tilde{\vct{l}}}
\providecommand{\dtvl}{\dot{\tilde{\vct{l}}}}
\providecommand{\vm}{\vct{m}}
\providecommand{\dvm}{\dot{\vct{m}}}
\providecommand{\tvm}{\tilde{\vct{m}}}
\providecommand{\dtvm}{\dot{\tilde{\vct{m}}}}
\providecommand{\vn}{\vct{n}}
\providecommand{\dvn}{\dot{\vct{n}}}
\providecommand{\tvn}{\tilde{\vct{n}}}
\providecommand{\dtvn}{\dot{\tilde{\vct{n}}}}
\providecommand{\vo}{\vct{o}}
\providecommand{\dvo}{\dot{\vct{o}}}
\providecommand{\tvo}{\tilde{\vct{o}}}
\providecommand{\dtvo}{\dot{\tilde{\vct{o}}}}
\providecommand{\vp}{\vct{p}}
\providecommand{\dvp}{\dot{\vct{p}}}
\providecommand{\tvp}{\tilde{\vct{p}}}
\providecommand{\dtvp}{\dot{\tilde{\vct{p}}}}
\providecommand{\vq}{\vct{q}}
\providecommand{\dvq}{\dot{\vct{q}}}
\providecommand{\tvq}{\tilde{\vct{q}}}
\providecommand{\dtvq}{\dot{\tilde{\vct{q}}}}
\providecommand{\vr}{\vct{r}}
\providecommand{\dvr}{\dot{\vct{r}}}
\providecommand{\tvr}{\tilde{\vct{r}}}
\providecommand{\dtvr}{\dot{\tilde{\vct{r}}}}
\providecommand{\vs}{\vct{s}}
\providecommand{\dvs}{\dot{\vct{s}}}
\providecommand{\tvs}{\tilde{\vct{s}}}
\providecommand{\dtvs}{\dot{\tilde{\vct{s}}}}
\providecommand{\vt}{\vct{t}}
\providecommand{\dvt}{\dot{\vct{t}}}
\providecommand{\tvt}{\tilde{\vct{t}}}
\providecommand{\dtvt}{\dot{\tilde{\vct{t}}}}
\providecommand{\vu}{\vct{u}}
\providecommand{\dvu}{\dot{\vct{u}}}
\providecommand{\tvu}{\tilde{\vct{u}}}
\providecommand{\dtvu}{\dot{\tilde{\vct{u}}}}
\providecommand{\vv}{\vct{v}}
\providecommand{\dvv}{\dot{\vct{v}}}
\providecommand{\tvv}{\tilde{\vct{v}}}
\providecommand{\dtvv}{\dot{\tilde{\vct{v}}}}
\providecommand{\vw}{\vct{w}}
\providecommand{\dvw}{\dot{\vct{w}}}
\providecommand{\tvw}{\tilde{\vct{w}}}
\providecommand{\dtvw}{\dot{\tilde{\vct{w}}}}
\providecommand{\vx}{\vct{x}}
\providecommand{\dvx}{\dot{\vct{x}}}
\providecommand{\tvx}{\tilde{\vct{x}}}
\providecommand{\dtvx}{\dot{\tilde{\vct{x}}}}
\providecommand{\vy}{\vct{y}}
\providecommand{\dvy}{\dot{\vct{y}}}
\providecommand{\tvy}{\tilde{\vct{y}}}
\providecommand{\dtvy}{\dot{\tilde{\vct{y}}}}
\providecommand{\vz}{\vct{z}}
\providecommand{\dvz}{\dot{\vct{z}}}
\providecommand{\tvz}{\tilde{\vct{z}}}
\providecommand{\dtvz}{\dot{\tilde{\vct{z}}}}
\providecommand{\vA}{\vct{A}}
\providecommand{\dvA}{\dot{\vct{A}}}
\providecommand{\tvA}{\tilde{\vct{A}}}
\providecommand{\dtvA}{\dot{\tilde{\vct{A}}}}
\providecommand{\vB}{\vct{B}}
\providecommand{\dvB}{\dot{\vct{B}}}
\providecommand{\tvB}{\tilde{\vct{B}}}
\providecommand{\dtvB}{\dot{\tilde{\vct{B}}}}
\providecommand{\vC}{\vct{C}}
\providecommand{\dvC}{\dot{\vct{C}}}
\providecommand{\tvC}{\tilde{\vct{C}}}
\providecommand{\dtvC}{\dot{\tilde{\vct{C}}}}
\providecommand{\vD}{\vct{D}}
\providecommand{\dvD}{\dot{\vct{D}}}
\providecommand{\tvD}{\tilde{\vct{D}}}
\providecommand{\dtvD}{\dot{\tilde{\vct{D}}}}
\providecommand{\vE}{\vct{E}}
\providecommand{\dvE}{\dot{\vct{E}}}
\providecommand{\tvE}{\tilde{\vct{E}}}
\providecommand{\dtvE}{\dot{\tilde{\vct{E}}}}
\providecommand{\vF}{\vct{F}}
\providecommand{\dvF}{\dot{\vct{F}}}
\providecommand{\tvF}{\tilde{\vct{F}}}
\providecommand{\dtvF}{\dot{\tilde{\vct{F}}}}
\providecommand{\vG}{\vct{G}}
\providecommand{\dvG}{\dot{\vct{G}}}
\providecommand{\tvG}{\tilde{\vct{G}}}
\providecommand{\dtvG}{\dot{\tilde{\vct{G}}}}
\providecommand{\vH}{\vct{H}}
\providecommand{\dvH}{\dot{\vct{H}}}
\providecommand{\tvH}{\tilde{\vct{H}}}
\providecommand{\dtvH}{\dot{\tilde{\vct{H}}}}
\providecommand{\vI}{\vct{I}}
\providecommand{\dvI}{\dot{\vct{I}}}
\providecommand{\tvI}{\tilde{\vct{I}}}
\providecommand{\dtvI}{\dot{\tilde{\vct{I}}}}
\providecommand{\vJ}{\vct{J}}
\providecommand{\dvJ}{\dot{\vct{J}}}
\providecommand{\tvJ}{\tilde{\vct{J}}}
\providecommand{\dtvJ}{\dot{\tilde{\vct{J}}}}
\providecommand{\vK}{\vct{K}}
\providecommand{\dvK}{\dot{\vct{K}}}
\providecommand{\tvK}{\tilde{\vct{K}}}
\providecommand{\dtvK}{\dot{\tilde{\vct{K}}}}
\providecommand{\vL}{\vct{L}}
\providecommand{\dvL}{\dot{\vct{L}}}
\providecommand{\tvL}{\tilde{\vct{L}}}
\providecommand{\dtvL}{\dot{\tilde{\vct{L}}}}
\providecommand{\vM}{\vct{M}}
\providecommand{\dvM}{\dot{\vct{M}}}
\providecommand{\tvM}{\tilde{\vct{M}}}
\providecommand{\dtvM}{\dot{\tilde{\vct{M}}}}
\providecommand{\vN}{\vct{N}}
\providecommand{\dvN}{\dot{\vct{N}}}
\providecommand{\tvN}{\tilde{\vct{N}}}
\providecommand{\dtvN}{\dot{\tilde{\vct{N}}}}
\providecommand{\vO}{\vct{O}}
\providecommand{\dvO}{\dot{\vct{O}}}
\providecommand{\tvO}{\tilde{\vct{O}}}
\providecommand{\dtvO}{\dot{\tilde{\vct{O}}}}
\providecommand{\vP}{\vct{P}}
\providecommand{\dvP}{\dot{\vct{P}}}
\providecommand{\tvP}{\tilde{\vct{P}}}
\providecommand{\dtvP}{\dot{\tilde{\vct{P}}}}
\providecommand{\vQ}{\vct{Q}}
\providecommand{\dvQ}{\dot{\vct{Q}}}
\providecommand{\tvQ}{\tilde{\vct{Q}}}
\providecommand{\dtvQ}{\dot{\tilde{\vct{Q}}}}
\providecommand{\vR}{\vct{R}}
\providecommand{\dvR}{\dot{\vct{R}}}
\providecommand{\tvR}{\tilde{\vct{R}}}
\providecommand{\dtvR}{\dot{\tilde{\vct{R}}}}
\providecommand{\vS}{\vct{S}}
\providecommand{\dvS}{\dot{\vct{S}}}
\providecommand{\tvS}{\tilde{\vct{S}}}
\providecommand{\dtvS}{\dot{\tilde{\vct{S}}}}
\providecommand{\vT}{\vct{T}}
\providecommand{\dvT}{\dot{\vct{T}}}
\providecommand{\tvT}{\tilde{\vct{T}}}
\providecommand{\dtvT}{\dot{\tilde{\vct{T}}}}
\providecommand{\vU}{\vct{U}}
\providecommand{\dvU}{\dot{\vct{U}}}
\providecommand{\tvU}{\tilde{\vct{U}}}
\providecommand{\dtvU}{\dot{\tilde{\vct{U}}}}
\providecommand{\vV}{\vct{V}}
\providecommand{\dvV}{\dot{\vct{V}}}
\providecommand{\tvV}{\tilde{\vct{V}}}
\providecommand{\dtvV}{\dot{\tilde{\vct{V}}}}
\providecommand{\vW}{\vct{W}}
\providecommand{\dvW}{\dot{\vct{W}}}
\providecommand{\tvW}{\tilde{\vct{W}}}
\providecommand{\dtvW}{\dot{\tilde{\vct{W}}}}
\providecommand{\vX}{\vct{X}}
\providecommand{\dvX}{\dot{\vct{X}}}
\providecommand{\tvX}{\tilde{\vct{X}}}
\providecommand{\dtvX}{\dot{\tilde{\vct{X}}}}
\providecommand{\vY}{\vct{Y}}
\providecommand{\dvY}{\dot{\vct{Y}}}
\providecommand{\tvY}{\tilde{\vct{Y}}}
\providecommand{\dtvY}{\dot{\tilde{\vct{Y}}}}
\providecommand{\vZ}{\vct{Z}}
\providecommand{\dvZ}{\dot{\vct{Z}}}
\providecommand{\tvZ}{\tilde{\vct{Z}}}
\providecommand{\dtvZ}{\dot{\tilde{\vct{Z}}}}

\providecommand{\vbeta}{\boldsymbol{\beta}}
\providecommand{\dvbeta}{\dot{\boldsymbol{\beta}}}
\providecommand{\vsigma}{\boldsymbol{\sigma}}
\providecommand{\dvsigma}{\dot{\boldsymbol{\sigma}}}

\providecommand{\te}{\tilde{e}}

% Shortand notation for derivatives and bold of symbols
\providecommand{\dgamma}{\dot{\gamma}}
\providecommand{\ddgamma}{\ddot{\gamma}}
\providecommand{\vgamma}{\bm{\gamma}}
\providecommand{\dDelta}{\dot{\Delta}}
\providecommand{\ddDelta}{\ddot{\Delta}}
\providecommand{\vDelta}{\bm{\Delta}}
\providecommand{\dpi}{\dot{\pi}}
\providecommand{\ddpi}{\ddot{\pi}}
\providecommand{\vpi}{\bm{\pi}}
\providecommand{\dvarphi}{\dot{\varphi}}
\providecommand{\ddvarphi}{\ddot{\varphi}}
\providecommand{\vvarphi}{\bm{\varphi}}

% Shortand notation for matrices
\providecommand{\mA}{\vct{A}}
\providecommand{\mB}{\vct{B}}
\providecommand{\mC}{\vct{C}}
\providecommand{\mD}{\vct{D}}
\providecommand{\mE}{\vct{E}}
\providecommand{\mF}{\vct{F}}
\providecommand{\mG}{\vct{G}}
\providecommand{\mH}{\vct{H}}
\providecommand{\mI}{\vct{I}}
\providecommand{\mJ}{\vct{J}}
\providecommand{\mK}{\vct{K}}
\providecommand{\mL}{\vct{L}}
\providecommand{\mM}{\vct{M}}
\providecommand{\mN}{\vct{N}}
\providecommand{\mO}{\vct{O}}
\providecommand{\mP}{\vct{P}}
\providecommand{\mQ}{\vct{Q}}
\providecommand{\mR}{\vct{R}}
\providecommand{\mS}{\vct{S}}
\providecommand{\mT}{\vct{T}}
\providecommand{\mU}{\vct{U}}
\providecommand{\mV}{\vct{V}}
\providecommand{\mW}{\vct{W}}
\providecommand{\mX}{\vct{X}}
\providecommand{\mY}{\vct{Y}}
\providecommand{\mZ}{\vct{Z}}

% Shortand notation for calligraphic upper case letters
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cH}{\mathcal{H}}
\providecommand{\cI}{\mathcal{I}}
\providecommand{\cJ}{\mathcal{J}}
\providecommand{\cK}{\mathcal{K}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cO}{\mathcal{O}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cQ}{\mathcal{Q}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cT}{\mathcal{T}}
\providecommand{\cU}{\mathcal{U}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cW}{\mathcal{W}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\cZ}{\mathcal{Z}}

% Shortand notation for some tilded symbols and their derivatives
\providecommand{\tx}{\tilde{x}}
\providecommand{\dtx}{\dot{\tilde{x}}}
\providecommand{\ty}{\tilde{y}}
\providecommand{\dty}{\dot{\tilde{y}}}
\providecommand{\tvarphi}{\tilde{\varphi}}
\providecommand{\dtvarphi}{\dot{\tilde{\varphi}}}



==> preamble/pagination.tex <==
\usepackage{cite}

%advanced typesetting
\usepackage{microtype}

% US hyphenation
\usepackage[american]{babel}


% extensions for tables
\usepackage{array}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{makecell} %introduces \thead and \makecell

%compact paragraph title
\newcommand{\myparagraph}[1]{\textbf{\emph{#1}}.}
%\newcommand{\subparagraph}[1]{\emph{#1}.}

%provide options for changing spacing in enumeration environments
\ifcsname labelindent\endcsname
\let\labelindent\relax
\fi
\usepackage[inline]{enumitem}

%provides subfloats (subcaption replaces subfig and subfigure, but
%might not be compatible with some classes)
\usepackage{subfig}

%Inspired by CVPR template
\providecommand{\ie}{i.e\onedot}
\newcommand{\eg}{e.g\onedot}
\providecommand{\etal}{et al\onedot}

%set more relaxed constraints on the floats
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{0.85}
\renewcommand{\textfraction}{0.15}
\renewcommand{\floatpagefraction}{0.7}

%Make an enumeration with a letter+progressive number
\newenvironment{lenumerate}[2][]
{\begin{enumerate}[label=(#2\arabic*),leftmargin=0.2in,itemindent=0.15in,#1]}
{\end{enumerate}}

%Make an letter+progressive number description list
\newenvironment{ldescription}[2][]
{\begin{lenumerate}{#2}%
\let\bitem\item%
\renewcommand{\item}[1][]{\bitem\textsl{##1}:~}}
{\end{lenumerate}}


 %The following sets the labeling for inline enumerations

\setlist*[enumerate,1]{label={\itshape\arabic*)}}

%Define macro to make paragraph headings always end with a full stop
\makeatletter
\newcommand{\paragraphswithstop}{%
\let\copyparagraph\paragraph%
\renewcommand\paragraph[1]{\copyparagraph{##1.}}%
}
\makeatother

%Package to frame text in boxes
\usepackage[framemethod=tikz]{mdframed}

% References by text instead of section or page number
\makeatletter
\def\namedlabel#1#2{\begingroup
  #2%
  \def\@currentlabel{#2}%
  \phantomsection\label{#1}\endgroup
}
\makeatother

%Same as above, but do not insert the label text
\makeatletter
\def\namedlabelphantom#1#2{\begingroup
  \def\@currentlabel{#2}%
  \phantomsection\label{#1}\endgroup
}
\makeatother

%Force exact termination of a paragraph with justification
\newcommand{\parunskip}{\bgroup\unskip\parfillskip=0pt \par\egroup}

%%% Local Variables:
%%% mode: latex
%%% End:


==> preamble/posterCommon.tex <==
\input{preamble/posterGraphics}
\input{preamble/posterFormatting}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterFormatting.tex <==
%fonts
\usepackage[scaled=0.90]{helvet}
\usepackage{courier}

%sectioning
\pagestyle{empty}
\setcounter{secnumdepth}{0}

%headings
\def\Head#1{\noindent\hbox to \hsize{\hfil{\veryHuge\color{DarkBlue} #1}}\bigskip}
\def\LHead#1{\noindent{\LARGE\color{Blue} #1}\vspace{-.5cm}}
\def\Subhead#1{\noindent{\Large\color{DarkBlue} #1}\vspace{-.5cm}}
\def\Subsubhead#1{{\color{Blue} #1}}
\def\Title#1{\noindent{\Huge #1}}

%text boxes and grid
%Note: use options showboxes if you want to see the boxes
\usepackage[absolute]{textpos}
\TPGrid[30mm,30mm]{10}{20}  % 3 - 1 - 7 - 1 - 3 Columns

% Mess with these as you like
\parindent=0pt
%\parindent=1cm
\parskip=0.5\baselineskip


==> preamble/posterGraphics.tex <==
\usepackage{tikz}
\usepackage{xcolor}

%colors
\definecolor{Blue}{rgb}{0.05,0.2,0.5}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{LightBlue}{rgb}{.2431,.5451,.8588}
\definecolor{Red}{rgb}{1.0,0,0}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}

%for callouts
\usetikzlibrary{calc,chains,positioning,shapes.callouts}

%bullet points
\renewcommand{\labelitemi}{\color{LightBlue}{$\bullet$}}

%highlighting
\newcommand{\alert}[1]{{\color{LightBlue} #1}}

%rounded boxes
\newenvironment{roundboxes}[1][]
{\begin{tikzpicture}[start chain,node distance=2cm,
 every node/.style={on chain, text=black,fill=LightBlue!20, rounded corners=0.6cm},#1]
}
{\end{tikzpicture}
}

%Define anchors for callouts
\newcommand{\anchor}[1]{\tikz[remember picture] \coordinate (#1);}

%Insert callouts. Syntax:
%\callout[optionalStyle]{pointer}{positionRelativeToThePointer}{text}
\newcommand{\callout}[4][]{\begin{tikzpicture}[remember picture, overlay]
 \node[rectangle callout, fill=gray!50, #1, callout absolute pointer={#2}] at ($ #2 + #3 $) {#4};
\end{tikzpicture}
}

%Rounded box to highlight plus define anchor
\newcommand{\enboxref}[3][]{
  \tikz[baseline,remember picture]{
    \node[fill=gray!20,anchor=base,rounded corners=0.6cm,#1] (#2) {#3};
  }
}

%Boxes to define sections
\newlength{\sectionboxpadding}
\setlength{\sectionboxpadding}{5mm}

\newcommand{\sectionboxcolor}{LightBlue}

\newcommand{\sectionboxstart}[1]{\makebox[0cm][l]{\anchor{#1 a}}}
\newcommand{\sectionboxend}[1]{\makebox[0cm][l]{\anchor{#1 b}} \vspace{-3em}\\}
\newcommand{\sectionboxdraw}[2][]{\begin{tikzpicture}[remember picture, overlay,#1]
 \draw[rounded corners, line width=5pt, draw=\sectionboxcolor] ($(#2 a)+(0,0.6em)+(-\sectionboxpadding,\sectionboxpadding)+(0,0.4em)$) rectangle ($(#2 b)+(\textwidth,1em)+(\sectionboxpadding,-\sectionboxpadding)+(0,0.4em)$);
\end{tikzpicture}
}

\newcommand{\generalboxdraw}{
\begin{tikzpicture}[remember picture, overlay, LightBlue]
\draw[line width=5pt] ($(current page.north west) + (2,-13.5)$) rectangle ($(current page.south east) + (-2,3)$);
\end{tikzpicture}
}


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

Use \var{\tikztestgrid{4}{3}} to draw, inside a \var{tikzpicture}, a test grid 4 units wide, 3 units tall, and centered at (0,0).

==> preamble/proposals.tex <==

\input{preamble/compactLists}
\input{preamble/proposalsPagination}
\input{preamble/proposalsFormatting}
\input{preamble/splitting}

\newcommand{\testgrid}{\tikz[remember picture, overlay]{%
  \coordinate (tl) at  ($(current page.north west)+(1in,-1in)$);%
  \coordinate (br) at  ($(current page.south east)+(-1in,1in)$);%
  \draw[red] (tl) rectangle (br);%
  \draw[red] (tl) grid[xstep=2\textwidth,ystep=1in] (br);}}




==> preamble/proposalsAggressive.tex <==
\linespread{0.93}


==> preamble/proposalsEnableHelvetica.tex <==
%These commands set Helvetica as the default font
\usepackage[scaled]{helvet}
\renewcommand\familydefault{\sfdefault} 
\usepackage[T1]{fontenc}


==> preamble/proposalsFormatting.tex <==
% For including the notes.org file
\input{preamble/formattingCode}

% Clever cross-references
\usepackage{cleveref}
% % Customize labels (see section 8.1.2 of cleveref's manual)
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{thrust}{Thrust}{Thrusts}
\Crefname{thrust}{Thrust}{Thrusts}
\crefname{section}{\S}{\S}
\Crefname{section}{\S}{\S}

\paragraphswithstop

% Reduce line skip before \paragraph
\titlespacing{\paragraph}{%
  0pt}{%              left margin
  0\baselineskip}{%   space before (vertical)
  0.5em}%             space after (horizontal)


% Change name of section for references
\renewcommand{\refname}{References Cited}

%Redefine \maketitle command
\makeatletter
\renewcommand{\maketitle}{\begin{center}\Large\textbf\@title
  \end{center}
  % Add author only if not empty (in the sense of producing output)
\setbox0=\hbox{\@author\unskip}\ifdim\wd0=0pt
\else
\begin{center}
  \@author
\end{center}
\fi%
}
\makeatother

%theorem-like environment for stating thrusts
%we define a second counter that is updated in synch with the default
%one, but is presented in Alphabetic form
\newtheorem{innerthrust}{Thrust}
\newcounter{thrustnumber}
\newenvironment{thrust}[1][\Alph{thrustnumber}]
  {\stepcounter{thrustnumber}\renewcommand\theinnerthrust{#1}\innerthrust}
  {\endinnerthrust}


%macros for paragraphs in thrust description
\newcommand{\thrustmerits}{\paragraph{Intellectual merits of
    this thrust}}
\WithSuffix\newcommand\thrustmerits*[1][\Alph{thrustnumber}]{\paragraph{Intellectual merits of thrust~#1}}

\newcommand{\thruststateoftheart}{\paragraph{State of
    the art and open problems}}
\WithSuffix\newcommand\thruststateoftheart*[1][\Alph{thrustnumber}]{\paragraph{Relation of thrust~#1 with the state of the art}}

\newcommand{\thrustbackground}[1]{\paragraph{Background on #1}}

\newcommand{\thrustgoal}{\paragraph{Goal of this thrust}}

\newcommand{\proposalcontribution}[1]{\paragraph{Proposed innovation: #1}}
\newcommand{\proposalfuturedirections}{\paragraph{Additional future directions}}

\newcommand{\thrustsubtitlesassubsections}{
\renewcommand{\proposalcontribution}[1]{\subsection{##1}}
\renewcommand{\proposalfuturedirections}{\subsection{Additional future directions}}
}

\newcommand{\collaborationletter}{\emph{Letter of collaboration}}

\setlist[description]{%
  font={\itshape}, % set the label font
}

% Adjust vertical spacing

% Ref: https://tex.stackexchange.com/questions/68408/remove-vertical-space-around-theorems
\makeatletter
\def\thm@space@setup{\thm@preskip=0pt\thm@postskip=0pt}
\newtheorem{remarknoskip}{Remark}
\makeatother

\setlength{\intextsep}{0em}

% Side remark boxes
\newenvironment{sideremark}[2][0.5\textwidth]{%
\wrapfigure{#2}{#1}\vspace{-3mm}

\mdframed
\remarknoskip
}{%
\endremarknoskip
\endmdframed
\endwrapfigure
}


==> preamble/proposalsNIH.tex <==
\input{preamble/proposalsEnableHelvetica}
\geometry{margin=0.5in}

==> preamble/proposalsPagination.tex <==
\usepackage{url}
\usepackage{times}

\usepackage[compact]{titlesec}

% Perfect 1 inch margins
\usepackage[letterpaper,margin=1in]{geometry}

%Make font for captions smaller (saves space and visually separates them from the main text)
\usepackage[font={footnotesize,sf}]{caption}

% Nice gantt charts
\usepackage{pgfgantt}



==> preamble/proposalsTaskSections.tex <==
%The following reformat the sections so that their labels read "Task x.y" instead of "x.y".
%Use the starred version of the command if you do not want this for
%some of the sections
\titleformat{\section}{\normalfont\large\bfseries}{Task \thesection:}{0.5ex}{}
\titleformat{\subsection}{\normalfont\bfseries}{Task \thesubsection:}{0.5ex}{}


==> preamble/proposalsTitles.tex <==
%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue4}\sffamily}

%Format titles
\titleformat*{\section}{\titlestyle \bfseries \Large}
\titleformat*{\subsection}{\titlestyle \bfseries \large}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}
\renewcommand{\paragraph}[1]{\par\noindent{\titlestyle\small\bfseries #1.~}}

% Format mdframed boxes
\mdfsetup{%
  middlelinecolor=DodgerBlue4,
  middlelinewidth=1pt,
  %backgroundcolor=red!10,
  roundcorner=3pt}

==> preamble/pysplitmaster <==
#!/usr/bin/env python
""" Script that splits the file master.pdf produced by the NSF Proposal template into the individual parts required for submissions """

import re
import subprocess
import icecream
from icecream import ic
from optparse import OptionParser


def main(options):
    baseFileName = options.filename

    # Open log file
    fileName = baseFileName + '.log'
    logFile = open(fileName, 'r')

    if options.verbose:
        ic(fileName)

    # Regexp for matching split markers
    reProg = re.compile(
        r'Split marker \[([\w\-]*)\] \[(start|end)\] \[(\d*)\]')

    # Check the log file line by line and add matches to list
    matchList = []
    for (lineNb, line) in enumerate(logFile):
        m = reProg.findall(line)
        if m:
            matchList += m
            if options.verbose:
                print('Match found on line', lineNb + 1, ':', m)

    if options.verbose:
        ic(matchList)

    # Transform the match list into a double dictionary
    matchDict = {}
    for m in matchList:
        if m[0] not in matchDict:
            matchDict[m[0]] = {}
        pageNumber = int(m[2])
        if m[1] == 'end':
            # Split marker gives +1 page for end. Fix that
            pageNumber -= 1
        matchDict[m[0]][m[1]] = pageNumber

    if not checkMatchDict(matchDict):
        return -1

    pdfFileName = baseFileName + '.pdf'

    for sectionName, v in matchDict.items():
        # Split a section in its own file
        cmd = [
            'pdftk', pdfFileName, 'cat',
            str(v['start']) + '-' + str(v['end']), 'output',
            sectionName + '.pdf'
        ]
        ic(cmd)
        subprocess.check_call(cmd)

        # Strip all annotations
        cmd = ['pdfStripAnnotations', sectionName + '.pdf']
        ic(cmd)
        subprocess.check_call(cmd)


def checkMatchDict(matchDict):
    ''' Checks consistency of starts/ends for match dictionary '''
    for k, v in matchDict.items():
        # check presence of start and end
        if 'start' not in v:
            print('Missing start for section ' + k)
            return False
        if 'end' not in v:
            print('Missing end for section ' + k)
            return False
        if v['end'] < v['start']:
            print('Start/end page numbers for section ' + k +
                  ' not consistent')
            return False
        return True


if __name__ == "__main__":
    parser = OptionParser()
    parser.add_option(
        "-f",
        "--master-file",
        dest="filename",
        help="base name of the master file to split without extension",
        default="master")
    parser.add_option("-v",
                      "--verbose",
                      action="store_true",
                      dest="verbose",
                      default=False,
                      help="print intermediate details")
    (options, args) = parser.parse_args()
    main(options)


==> preamble/reviewDraft.tex <==
\usepackage{background}
\backgroundsetup{contents={%
    \begin{tikzpicture}[overlay,font=\sffamily]
      % \newcommand{\scaletop}{-.68in}
      % \newcommand{\scalepitch}{1.15em}
      % \newcommand{\scaleoffset}{.5in}
      % \foreach \x in {1,...,60}{
      %   \node at ($(current page.north west)+(\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+\x)}\pgfmathresult};
      %   \node at ($(current page.north east)+(-\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+100+\x)}\pgfmathresult};
      % }
      \node at ($(current page.south)+(0,.5in)$) {*** For Review Only ***};
    \end{tikzpicture}
  },color=blue,scale=1,angle=0}
\let\bframe\relax %remove command from robotics.tex conflicting with lineno
\usepackage[displaymath, mathlines,switch]{lineno}
\linenumbers
\author{\textcolor{blue}{\sffamily Author Names Omitted for Anonymous Review}}
\renewcommand{\author}[1]{}


==> preamble/robotics.tex <==
\tikzset{ax/.style={-latex,line width=2pt}}
\newcommand{\ax}[5][]{\begin{scope}[xshift=#3,yshift=#4,rotate=#5]%
    \node at (-0.3,-0.3) {$#1$};%
    \coordinate (ax#2o) at (0,0);%
    \draw[ax] (0,0) -- (1,0) node[pos=1.2] (ax#2a) {};%
    \draw[ax] (0,0) -- (0,1) node[pos=1.2] (ax#2b) {};%
  \end{scope}}

\newcommand{\axlabels}[3]{\node at (ax#1a) {$#2$};
  \node at (ax#1b) {$#3$};
}
\newcommand{\axup}[3][0]{\begin{scope}[rotate=#1]
\fill[ax] (ax#2o) circle[radius=3pt];
\path (ax#2o) ++(0.25,-0.25) node{$#3$};
\end{scope}
}
\newcommand{\axdown}[3]{\begin{scope}[rotate=#3]
    \draw[line width=2pt] (ax#1o) +(-3pt,-3pt) -- +(3pt,3pt) +(-3pt,3pt) -- +(3pt,-3pt);
    \path (ax#1o) ++(0.25,-0.25) node{$#2$};
  \end{scope}
}

\newcommand{\gpoint}[3][0]{\fill[ax] (#2) circle[radius=3pt];
  \path (#2) ++(#1:0.4) node[ax]{$#3$};
}

\tikzset{camera/.style={fill=Sienna1,fill opacity=0.5},%
image plane/.style={draw=RoyalBlue3,line width=2pt}}
\newcommand{\camera}[5][]{\begin{scope}[xshift=#3,yshift=#4,rotate=#5]
\ax[#1]{#2}{0}{0}{0}
\draw[image plane] (-1.2,1) -- (1.2,1);
\draw[camera] (0,0) -- (0.5,0.5) -- (-0.5,0.5) -- cycle; 
\end{scope}}

\newcommand{\gridworld}{\draw[gray] (0,0) grid[step=1cm] (5,5);}

\newcommand{\wframe}{\prescript{w}{}}
\newcommand{\Wframe}{\prescript{\cW}{}}
\newcommand{\iframe}{\prescript{i}{}}
\newcommand{\jframe}{\prescript{j}{}}
\newcommand{\bframe}[1][]{\prescript{b_{#1}}{}}
\newcommand{\Bframe}[1][]{\prescript{\cB_{#1}}{}}

\newcommand{\BtoWpose}{(\Wframe R_\cB,\Wframe T_\cB)}
\newcommand{\BtoWrot}{\Wframe R_\cB}
\newcommand{\BtoWtransl}{\Wframe T_\cB}
\newcommand{\BtoWposeVel}{(\Wframe{}\dot{R}_\cB,\Wframe{}\dot{T}_\cB)}
\newcommand{\BtoWrotVel}{\Wframe{}\dot{R}_\cB}
\newcommand{\BtoWtranslVel}{\Wframe{}\dot{T}_\cB}

\newcommand{\WtoBpose}{(\Bframe R_\cW,\Bframe T_\cW)}
\newcommand{\WtoBrot}{\Bframe R_\cW}
\newcommand{\WtoBtransl}{\Bframe T_\cW}
\newcommand{\WtoBposeVel}{(\Bframe{}\dot{R}_\cW,\Bframe{}\dot{T}_\cW)}
\newcommand{\WtoBrotVel}{\Bframe{}\dot{R}_\cW}
\newcommand{\WtoBtranslVel}{\Bframe{}\dot{T}_\cW}

\newcommand{\Bframex}{\Bframe x}
\newcommand{\Wframex}{\Wframe x}

% shorthand notation for 2-D rotation written as function of theta
\newcommand{\rottheta}{\left[ \begin{smallmatrix}
    \cos(\theta) & -\sin(\theta)\\ \sin(\theta) & \cos(\theta)
  \end{smallmatrix}
\right]}

%names of path planning algorithms
\newcommand{\rrt}{$\mathtt{RRT}$}
\newcommand{\rrtstar}{$\mathtt{RRT^*}$}
\newcommand{\astar}{$\mathtt{A^*}$}


==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}


==> preamble/splitting.tex <==
% Package to get PDF page numbers via \theCurrentPage
\usepackage{pageslts}
\pagenumbering{arabic}

% Macro to reset a counter to zero if it is defined
% Source: adapted from https://tex.stackexchange.com/questions/155776/check-if-counter-exists
\makeatletter
\newcommand*\resetcounter[1]{%
\ifcsname c@#1\endcsname % Check that counter exists
\setcounter{#1}{0}
\fi
}
\makeatother

% Macro to include file while writing to log file the splitting markers
\newenvironment{markforsplit}[1]{%
\def\splitmarkername{#1}
\typeout{Split marker [#1] [start] [\theCurrentPage]}  \setcounter{page}{1}%
\resetcounter{figure}
\resetcounter{table}
}{%
\clearpage%
\typeout{Split marker [\splitmarkername] [end] [\theCurrentPage]}%
}
\newcommand{\includeforsplit}[1]{%
\begin{markforsplit}{#1}%
\include{#1}%
\end{markforsplit}%
}


==> preamble/thesis.tex <==
% Additional settings and packages for the BU thesis
\usepackage[utf8]{inputenc}

% formatting

% set font to times new roman
\usepackage{newtxtext,newtxmath}

% set font size for headings
\usepackage{sectsty}
\chapterfont{\Large}
\sectionfont{\normalsize}
\subsectionfont{\normalsize}
% \allsectionsfont{\normalsize} % uncomment if you want all headings normal size

% set margins
\usepackage[letterpaper, top=1.5in, left=1.5in, right=1in, bottom=1in]{geometry}

% sets label font in captions to bold font
\usepackage[labelfont=bf]{caption}

% set hyperreferences
% \usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor= [rgb]{0.03, 0.44, 0.67},
    citecolor= [rgb]{0.03, 0.44, 0.67},
    linktocpage = true,
    bookmarks=true,
    urlcolor=cyan,
}

% set double spacing
\usepackage{setspace}
\doublespacing

% set single spacing in subequations enviornment
\BeforeBeginEnvironment{subequations}{\begin{singlespace}}
\AfterEndEnvironment{subequations}{\end{singlespace}\noindent\ignorespaces}

% set single spacing in equation enviornment
\BeforeBeginEnvironment{equation}{\begin{singlespace}}
\AfterEndEnvironment{equation}{\end{singlespace}\noindent\ignorespaces}

% set single spacing in align enviornment
\BeforeBeginEnvironment{align}{\begin{singlespace}}
\AfterEndEnvironment{align}{\end{singlespace}\noindent\ignorespaces}

% set single spacing in lstlisting enviornment
\BeforeBeginEnvironment{lstlisting}{\begin{singlespace}}
\AfterEndEnvironment{lstlisting}{\end{singlespace}\noindent\ignorespaces}


% additional packages

\usepackage{longtable} % table span multiple pages
\usepackage{tcolorbox} % framed color box
\usepackage{lscape,afterpage} % landscape pages
\usepackage{listings} % codes
\lstset{escapeinside={<@}{@>}} % command to escape within lstlisting


% description w/out bold font
% \setlist[description]{font=\normalfont}

% the header is empty and the footer contains page numbers in the centre
\pagestyle{plain}


==> preamble/units.tex <==
%command for units of measure
\usepackage{units}

%S.I. units for some standard quantities
\newcommand{\upos}[1][]{\unit[#1]{m}}
\newcommand{\urad}[1][]{\unit[#1]{rad}}
\newcommand{\uvel}[1][]{\unitfrac[#1]{m}{s}}
\newcommand{\uacc}[1][]{\unitfrac[#1]{m}{s^2}}
\newcommand{\uavel}[1][]{\unitfrac[#1]{rad}{s}}
\newcommand{\uaacc}[1][]{\unitfrac[#1]{rad}{s^2}}
\newcommand{\uforce}[1][]{\unit[#1]{N}}
\newcommand{\utime}[1][]{\unit[#1]{s}}
\newcommand{\umass}[1][]{\unit[#1]{kg}}
\newcommand{\uspring}[1][]{\unitfrac[#1]{N}{m}}
\newcommand{\udamping}[1][]{\unitfrac[#1]{N\cdot s}{m}}
\newcommand{\ulength}[1][]{\unit[#1]{m}}
\newcommand{\uinertia}[1][]{\unit[#1]{kg\cdot m^2}}


==> preamble/utilities.tex <==
% Allow easy definition of starred version of commands
% Ref: https://tex.stackexchange.com/questions/202504/macro-to-add-starred-version-of-command
\usepackage{suffix}

% Allow definition of environments with extra final code
\usepackage{environ}

% Define warning sign by extracting it from the Fourier package
% Source: https://tex.stackexchange.com/questions/159669/how-to-print-a-warning-sign-triangle-with-exclamation-point
\newcommand{\danger}{\textcolor{red}{\fontencoding{U}\fontfamily{futs}\selectfont\char49\relax}}

% Insert a prefix-argument-postfix text only if argument is non-empty
% Needs to use a savebox to avoid evaluating the argument multiple times
\makeatletter
\newsavebox{\boxifnotempty}
\newcommand{\displayifnotempty}[3]{\sbox\boxifnotempty{#2}\setbox0=\hbox{\usebox{\boxifnotempty}\unskip}%
  \ifdim\wd0=0pt
  \else
  #1\usebox{\boxifnotempty}#3%
  \fi%
}

% \ifempty{1}{2} displays 2 if 1 is empty
\newcommand{\ifempty}[2]{\setbox0=\hbox{#1\unskip}%
  \ifdim\wd0=0pt%
  #2%
  \fi%
}

% \ifnotempty{1}{2} displays 2 if 1 is not empty
\newcommand{\ifnotempty}[2]{\setbox0=\hbox{#1\unskip}%
  \ifdim\wd0>0pt%
  #2%
  \fi%
}
\makeatother

% \switchempty{1}{2}{3} displays 2 if 1 is empty, otherwise 3
\newcommand{\switchifempty}[3]{\sbox\boxifnotempty{#1}\setbox0=\hbox{\usebox{\boxifnotempty}\unskip}%
  \ifdim\wd0=0pt{}%
  #2%
  \else{}%
  #3%
  \usebox{\boxifnotempty}%
  \fi%
}


% introduce the algorithmic environment and the algorithm floats
\makeatletter
\@ifundefined{chapter}{\usepackage{algorithm}}{\usepackage[chapter]{algorithm}}
\makeatother
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\makeatother%

% macros for storing definitions across compilations
\usepackage{scrlfile}

\makeatletter
%mark a definition to be stored in the aux file
\newcommand*\newstoreddef[1]{
  \BeforeClosingMainAux{%
    \immediate\write\@auxout{%
      \string\restoredef{#1}{\csname #1\endcsname}%
    }%
  }%
}
%used by the aux file to restore the definition
\newcommand*{\restoredef}[2]{% used at the aux file
  \expandafter\gdef\csname stored@#1\endcsname{#2}%
}
%show the stored definition (user command to ask for the value)
\newcommand*{\storeddef}[1]{
  \@ifundefined{stored@#1}{0}{\csname stored@#1\endcsname}%
}
\makeatother

%Add values to non-counter definitions (works with non-integers)
\newcommand{\addtovar}[2]{\pgfmathparse{#1+#2}\xdef#1{\pgfmathresult}}
\newcommand{\zerovar}[1]{\xdef#1{0}}

%Insert content of a PGF variable
\newcommand{\pgfprint}[1]{\pgfmathparse{#1}\pgfmathresult}

%Package to get PDF page numbers
\usepackage{pageslts}
\pagenumbering{arabic}

%Output content of enviroment both to the document and to the log file
%In the log file, the content is marked by start/end delimiters, and
%macros are not expanded.
\NewEnviron{tee}{\BODY\typeout{Marker Tee [start] ^^J \BODY ^^JMaker Tee [end]}}


%%% Local Variables:
%%% mode: latex
%%% End:


==> preamble/video.tex <==
\usepackage[bigfiles]{pdfbase}
\ExplSyntaxOn
%%begin novalidate
\cs_new:Npn\embedvideo#1#2{
%%end novalidate
  \leavevmode
  \pbs_pdfobj:nnn{}{fstream}{{}{#2}}
  \pbs_pdfobj:nnn{}{dict}{
    /Type/Filespec/F~(#2)/UF~(#2)
    /EF~<</F~\pbs_pdflastobj:>>
  }
  \tl_set:Nx\video{\pbs_pdflastobj:}%
  %
  \pbs_pdfobj:nnn{}{dict}{
    /Type/RichMediaInstance/Subtype/Video
    /Asset~\video
    /Params~<</Binding/Foreground>>
  }
  %
  \pbs_pdfobj:nnn{}{dict}{
    /Type/RichMediaConfiguration/Subtype/Video
    /Instances~[\pbs_pdflastobj:]
  }
  %
  \pbs_pdfobj:nnn{}{dict}{
    /Type/RichMediaContent
    /Assets~<<
      /Names~[(#2)~\video]
    >>
    /Configurations~[\pbs_pdflastobj:]
  }
  \tl_set:Nx\rmcontent{\pbs_pdflastobj:}%
  %
  \pbs_pdfobj:nnn{}{dict}{
    /Activation~<<
      /Condition/XA
      /Presentation~<<
        /Transparent~true
        /Style/Embedded
        /PassContextClick~true
      >>
    >>
    /Deactivation~<</Condition/PC>>
  }
  %
  \hbox_set:Nn\l_tmpa_box{#1}
  \tl_set:Nx\l_box_wd_tl{\dim_use:N\box_wd:N\l_tmpa_box}
  \tl_set:Nx\l_box_ht_tl{\dim_use:N\box_ht:N\l_tmpa_box}
  \tl_set:Nx\l_box_dp_tl{\dim_use:N\box_dp:N\l_tmpa_box}
  \pbs_pdfxform:nnnnn{1}{1}{}{}{\l_tmpa_box}
  %
  \pbs_pdfannot:nnnn{\l_box_wd_tl}{\l_box_ht_tl}{\l_box_dp_tl}{
    /Subtype/RichMedia
    /BS~<</W~0/S/S>>
    /Contents~(embedded~video~file:#2)
    /NM~(rma:#2)
    /AP~<</N~\pbs_pdflastxform:>>
    /RichMediaSettings~\pbs_pdflastobj:
    /RichMediaContent~\rmcontent
  }
  \phantom{#1}
}%
\ExplSyntaxOff

% Example use: \embedvideo{<poster or text>}{<video file (MP4+H264)>}

